Neuro-symbolic Natural Logic with Introspective Revision for Natural Language Inference

We introduce a neuro-symbolic natural logic framework based on reinforcement learning with introspective revision. The model samples and rewards specific reasoning paths through policy gradient, in which the introspective revision algorithm modifies intermediate symbolic reasoning steps to discover reward-earning operations as well as leverages external knowledge to alleviate spurious reasoning and training inefficiency. The framework is supported by properly designed local relation models to avoid input entangling, which helps ensure the interpretability of the proof paths. The proposed model has built-in interpretability and shows superior capability in monotonicity inference, systematic generalization, and interpretability, compared to previous models on the existing datasets.

==> backup/backup.tex <==
Download

Source

PDF
Actions
   Copy Project
   Word Count
Sync
   Dropbox
   Git
   GitHub
Settings
Compiler

pdfLaTeX
TeX Live version

2020
Main document

tacl2018v2-template.tex
Spell check

English
Auto-complete

On
Auto-close Brackets

On
Code check

On
Editor theme

textmate
Overall theme

Default
Keybindings

None
Font Size

16px
Font Family

Lucida / Source Code Pro
Line Height

Normal
PDF Viewer

Built-In
Help
   Show Hotkeys
   Documentation
   Contact Us
Back to your projects
Natlogic

File outline
Introduction

Related Work
Natural Logic.
Natural Language Inference.
Combine Neural Network with Natural Logic.
Background

Method

Neuro-Symbolic Natural Logic Model
Encoding and Phrase Representation.
Local Relations.
Natural Logic Program.
Rewards and Optimization.
Data Augmentation.

Introspective Revision Algorithm
Lexical Knowledge.
Algorithm.

Experiments

Performance on Monotonicity Reasoning
Dataset.
Systematicity of Monotonicity Inference
Model Explanation
Case Study
Conclusion
Editor mode.
 
  \textbf{GPT-2}~\cite{gpt2} & 89.5   &   52.1   &  44.8   &   57.5 & 48.3\\


 

5 warnings

